KITRO: Refining Human Mesh by 2D Clues and Kinematic-tree Rotation

2D keypoints are commonly used as an additional cue to refine estimated 3D human meshes. Current methods optimize the pose and shape parameters with a reprojection loss on the provided 2D keypoints. Such an approach, while simple and intuitive, has limited effectiveness because the optimal solution is hard to find in ambiguous parameter space and may sacrifice depth. Additionally, divergent gradients from distal joints complicate and deviate the refinement of proximal joints in the kinematic chain. To address these, we introduce Kinematic-Tree Rotation (KITRO), a novel mesh refinement strategy that explicitly models depth and human kinematic-tree structure. KITRO treats refinement from a bone-wise perspective. Unlike previous methods which perform gradient-based optimizations, our method calculates bone directions in closed form. By accounting for the 2D pose, bone length, and parent joint's depth, the calculation results in two possible directions for each child joint. We then use a decision tree to trace binary choices for all bones along the human skeleton's kinematic-tree to select the most probable hypothesis. Our experiments across various datasets and baseline models demonstrate that KITRO significantly improves 3D joint estimation accuracy and achieves an ideal 2D fit simultaneously. Our code available at: https://github.com/MartaYang/KITRO.

==> sec/x_suppl_bkup.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

% Reset the section counter
\setcounter{section}{0}
% Redefine the section numbering to use letters
\renewcommand{\thesection}{\Alph{section}}

\section{Details on Swing-Twist Decomposition} \label{supp:swingtwist}

\section{Proof-of-concept for Solution Selection} \label{supp:proofofconcept}

\section{Correctness Proof for \cref{eq:thetaupdating}} \label{supp:proof}

\section{More Ablation Studies} \label{supp:moreablation}

\section{Visulization of Samples Improvement Distribution} \label{supp:Distribution}

\section{Names of Joints and Bones on Kinematic-tree} \label{supp:nameKT}



\section{More Implementation Details}
Kinematic Tree. List all the bone that we are using.

Evaluation Metric: all neutral gender; include hard samples; average of 2 hips as base joint

\todo{alignment of 2dkp; }

Since we use Adam optimizer optimizer, we also perform ablation study on how 


\todo{2d repro error; (rewind)}

\section{fully experiments}

\begin{table*}[t!]
    \centering
    \caption{Camera}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        KAR w/o CE & 28.53 & 46.68 & 57.76     & & 21.30 & \textbf{33.22} & \textbf{41.12}\\
        KAR w/o Eq.\ref{eq:cammovingavg} & 27.99 & 50.21 & 61.11     & & 21.21 & 37.49 & 46.59\\
        \hline
        KAR  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & 34.50 & 42.88\\
        \hline
    \end{tabular}
    \label{tab:allcam}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{Shape}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        KAR w/o SO & 35.00 & 69.02 & 84.25     & & 35.40 & 55.01 & 66.18\\
        2D reproj. loss & 32.60 & 52.60 & 64.45     & & 30.38 & 50.32 & 62.41\\
        \hline
        KAR  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:allshape}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{Shape iteration number}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        iter 100  & 31.30 & 46.84 & 58.78     & &  &  & \\
        iter 50  & 29.36 & 44.12 & 54.68     & &  &  & \\
        iter 40  & 28.79 & 43.34 & 53.51     & &  &  & \\
        iter 30  & 28.15 & 42.34 & 52.09     & &  &  & \\
        iter 20  & 27.56 & 42.07 & 51.55     & &  &  & \\
        iter 10  & 27.67 & 43.53 & 53.44     & &  &  & \\
        iter 5 & 28.57 & 47.31 & 58.74     & &  &  & \\
        iter 1 & 34.91 & 69.24 & 81.99     & &  &  & \\
        iter 0 & 43.76 & 73.67 & 91.58     & &  &  & \\
        \hline
        KAR (iter 10)  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:shapeiter}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{Shape learning rate}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        lr 1.0  & 38.29 & 61.78 & 76.17     & &  &  & \\
        lr 0.5  & 31.68 & 49.26 & 60.33     & &  &  & \\
        lr 0.2  & 28.23 & 43.47 & 53.00     & &  &  & \\
        lr 0.1  & 27.67 & 43.53 & 53.44     & &  &  & \\
        lr 0.05  & 28.25 & 47.78 & 58.90     & &  &  & \\
        lr 0.01 & 32.71 & 63.59 & 76.75     & &  &  & \\
        \hline
        KAR (lr 0.1)  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:shapeiter}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{Pose}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        KAR w/o PR & 44.57 & 80.03 & 95.71     & & 37.98 & 65.54 & 83.60\\
        KAR w/o DecisionTree & 28.78 & 44.52 & 54.43     & & 21.61 & 34.93 & 43.34\\
        KAR w/o rewind & 28.10 & 44.39 & 54.27     & & 21.46 & 35.06 & 43.37\\
        KAR w/o reweighting & 32.18 & 52.15 & 63.82     & & 24.10 & 40.23 & 48.45\\
        \hline
        KAR  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:allpose}
\end{table*}


\begin{table*}[t!]
    \centering
    \caption{Loop number}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        loop 50  & 29.08 & 45.89 & 56.53     & &  &  & \\
        loop 20  & 27.83 & 43.35 & 53.37     & &  &  & \\
        loop 5  & 27.76 & 44.05 & 54.09     & &  &  & \\
        loop 1 & 33.05 & 53.37 & 66.36     & &  &  & \\
        loop 0 (baseline) & 43.0 & 69.0 & 81.2     & & 36.16 & 55.18 & 74.46\\
        \hline
        KAR (loop 10)  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:loopnum}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{SOTA comparision on 3DPW and HM36. (*) denotes the result of ours reproduction.}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        Baseline (report) & 43.0 & 69.0 & 81.2     & & - & - & - \\
        Baseline (w/o GT2D) & 43.76 & 73.67 & 91.58     & & 36.16 & 55.18 & 74.46 \\
        \hline 
        DynaBOA & 40.4 & 65.5 & 82.0    & & - & - & -\\
        Pose2Mesh & 34.6 & 65.1 & -     & & 35.3 & 51.1 & -\\
        CLIFF (w/ GT2D) diff.criterion  & 32.8 & 52.8 & 61.5      & & - & - & -\\
        CLIFF* (w/ GT2D 3DPW) & 32.04 & 55.83 & 71.95      & & 36.16 & 55.18 & 74.46\\
        CLIFF* (w/ GT2D HM36) & 46.17 & 77.85 & 94.71      & & 25.88 & 42.79 & 60.60\\
        CLIFF+SMPLify* & 32.63 & 58.89 & 75.90      & & 28.71 & 45.62 & 63.77\\
        \hline
        KAR \textbf{(Ours)}  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
        KAR (Ours on CLIFF 3DPW)  & 26.21 & 46.96 & 57.53      & & 25.14 & 41.75 & 51.67\\
        KAR (Ours on CLIFF HM36)  & 28.22 & 44.35 & 54.38      & & 20.28 & 34.77 & 43.37\\
        \hline
        SPIN-baseline  & 59.97 & 102.12 & 130.62      & & 40.57 & 61.65 & 83.61\\
        SPIN\textbf{+ours}  & 42.46 & 67.12 & 80.25      & & 26.45 & 37.91 & 47.46\\
        SPIN+SMPLify* & 43.64(47.99) & 79.56(87.06) & 101.50(102.28)      & &  &  & \\
        \hline
        EFT-baseline  & 54.71 & 94.02 & 116.23      & & 44.54 & 68.00 & 89.43\\
        EFT\textbf{+ours}  & 32.34 & 49.14 & 59.28      & & 26.24 & 41.17 & 49.68 \\
        \hline
    \end{tabular}
    \label{tab:SOTA}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{Upper-bound study}
    \begin{tabular}{lccccccc}
        \hline 
        & \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 2 - 4 } \cline { 6 - 8 }
        Method & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        % GT intrinsic  & 29.08 & 45.89 & 56.53     & &  &  & \\
        GT camera translation  &  &  &      & &  &  & \\
        \hline
        GT shape  &  &  &      & &  &  & \\
        \hline
        GT hypothesis &  &  &      & &  &  & \\
        \hline
        KAR (loop 10)  & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:loopnum}
\end{table*}

\begin{table*}[t!]
    \centering
    \caption{Upper-bound study}
    \begin{tabular}{cccccccccc}
        \hline 
        &&& \multicolumn{3}{c}{3DPW} & & \multicolumn{3}{c}{Human3.6M} \\
        \cline { 4 - 6 } \cline { 8 -  10}
        Camera & Shape & Pose & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ & & PA-MPJPE $\downarrow$ & MPJPE $\downarrow$ & PVE $\downarrow$ \\
        \hline 
        \ding{55} & \ding{55} & \ding{55} & 43.76 & 73.67 & 91.58     & & 36.16 & 55.18 & 74.46 \\
        \checkmark  & \ding{55} & \ding{55} & 43.76 & 73.67 & 91.58     & & 36.16 & 55.18 & 74.46\\
        \ding{55} & \checkmark & \ding{55}  & 44.31 & 69.92 & 83.26     & & 37.74 & 54.02 & 67.94\\        
        \ding{55} & \ding{55} &  \checkmark & 45.92 & 87.33 & 100.73     & & 34.87 & 52.63 & 68.09\\
        \checkmark & \checkmark  & \ding{55} & 44.57 & 80.03 & 95.71     & & 37.98 & 65.54 & 83.60\\
        \checkmark & \ding{55} & \checkmark & 35.00 & 69.02 & 84.25     & & 35.40 & 55.01 & 66.18\\
        \ding{55} & \checkmark & \checkmark  & 28.53 & 46.68 & 57.76     & & 21.30 & 33.22 & 41.12\\
        \checkmark & \checkmark & \checkmark & \textbf{27.67} & \textbf{43.53} & \textbf{53.44}      & & \textbf{21.04} & \textbf{34.50} & \textbf{42.88}\\
        \hline
    \end{tabular}
    \label{tab:allpose}
\end{table*}

% \section{Rationale}
% \label{sec:rationale}
% % 
% Having the supplementary compiled together with the main paper means that:
% % 
% \begin{itemize}
% \item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
% \item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
% \item When submitted to arXiv, the supplementary will already included at the end of the paper.
% \end{itemize}
% % 
% To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.
